Topics in Magnetic Geometry: Interpolation, Intersections and Integrability

This paper develops new links between contact geometry, magnetic dynamics, and symmetry in exact magnetic systems. First, we establish an interpolation property for Killing magnetic systems on contact manifolds under an additional condition. Specifically, we show that the corresponding magnetic geodesic flow interpolates smoothly between the sub-Riemannian geodesic flow on the contact distribution and the flow of the vector field associated with a primitive of the magnetic field. Second, we show that Hamiltonian group actions associated with the magnetomorphism group produce Poisson-commuting integrals of motion for the magnetic flow. Finally, we obtain new structural results on totally magnetic submanifolds, showing that fixed-point sets of magnetomorphisms and intersections of totally magnetic submanifolds are again totally magnetic. The latter two results may be viewed as extensions of classical phenomena from Riemannian geometry to magnetic geometry.

==> Sections/Interpolation.tex <==
\todolevin{add overview and explain aim of subsection}

In this subsection, we illustrate that condition \ref{it:th hyp} in \Cref{t: main theorem} is related to a so-called \emph{interpolation property}\marginpar{\lina{maybe need to reformulate, see how intro goes}}, which is of independent interest. This property concerns the angle between the vector field \( X \)\marginpar{\lina{same, introduce}} and the Reeb direction \( \R \) along magnetic geodesics, and is closely related to whether the norm of \( X \) remains constant along these orbits, as we explain in \Cref{r: relation (a) and (a')}. If we strengthen this condition to hold along all orbits of the magnetic geodesic flow, it implies the interpolation property for Killing magnetic systems. This property generalizes~\cite[Cor.~1.8]{ABM}.

\begin{thm}\label{prop: general interpolation}
Let \((M^{2n+1}, \alpha)\) be a closed contact manifold equipped with a Riemannian metric \(g\), and suppose that the magnetic system \((M, g, \mathrm{d}\alpha)\) is Killing.  Assume  that for the $g$-metric dual $X$ of $\alpha$ it holds:
\begin{equation}
    X_p\in \ker \d\alpha_p \quad \forall p\in M\, .
\end{equation}
Then the magnetic geodesic flow \( \varPhi_{g, \mathrm{d}\alpha} \) of the system \( (M, g, \mathrm{d}\alpha) \) interpolates smoothly between the sub-Riemannian geodesic flow on the distribution \( \xi := \ker \alpha \) and the flow of \( X \). 

More specifically:
\begin{enumerate}
    \item \label{it:prop sR}If \( \gamma \) is a magnetic geodesic with initial velocity \( \dot{\gamma}(0) \in \xi \), then \( \gamma \) is a sub-Riemannian geodesic tangent to the distribution \( \xi \).
    
    \item \label{it:prop 'Reeb'}If \( \gamma \) is a magnetic geodesic with initial velocity \( \dot{\gamma}(0) = r \cdot X_{\gamma(0)} \) for some \( r \in \mathbb{R} \), then \( \gamma \) is a reparameterization of a flow line of the vector field \( r \cdot X \).
\end{enumerate}
\end{thm}
\todolevin{I would add that $g_{\gamma}(X_{\gamma}, \dot{\gamma})$ is a conserved quantity to the statement}
\begin{comment}
    
\begin{rem}\label{r: relation (a) and (a')}
Condition \ref{it:prop hyp}, in combination with the assumption that the flow of \(X\) has at least \(n\) periodic orbits implies \ref{it:th hyp}. However, condition \ref{it:th hyp} does not always imply \ref{it:prop hyp} as can been seen for example in the setting of \Cref{cor: contact tpe property ellipsoids}.\marginpar{\lina{reformulate remarks}}
\end{rem}
\begin{rem}\label{r:flow_lines_of_rX_are_magnetic_geodesics}
Conversely, the implications in (1) and (2) also hold in reverse, where one has to suppose in addition to $(1)$ that \ref{it:prop hyp} holds.
To clarify the case of greatest interest to us: if \(\gamma\) is a flow line of \(r \cdot X\) for some \(r \in \mathbb{R}\), then \(\gamma\) is a magnetic geodesic in \((M, g, \mathrm{d}\alpha)\). This follows immediately from the proof of the key \Cref{l: key lemma}.
\end{rem}
\begin{rem}
Note that one can derive the existence statement in part (\ref{it:th neg action}) of \Cref{t: main theorem}-that is, the existence of at least \(n\) periodic orbits and \(n_0\) contractible ones of prescribed energy \(\kappa\) for each \(\kappa \in (0, \infty)\)—from \Cref{prop: general interpolation} under the following alternative assumption: \textit{“The sub-Riemannian geodesic flow of \((M, \ker \alpha = \xi)\) has \(n \in \mathbb{N} \cap [1, \infty]\) periodic orbits of the flow of \(X\), among which \(0 \leq n_0 \leq n\) are contractible.”} Under this assumption, the conclusion of part (\ref{it:th neg action}) still holds as a statement about existence on each energy level. However, since these sub-Riemannian geodesics have positive action, this setting does not allow one to deduce part (2) of \Cref{t: main theorem}, which relies crucially on the orbits having negative action (as ensured by condition \ref{it:th hyp}. The assumption above is always satisfied for \(n = 1\) if the unit sphere bundle \(T^1M\), equipped with its canonical contact structure, admits a so-called \emph{Plastikstufe}, as shown in \cite{albers2009weinstein}.
\end{rem}
\end{comment}


\begin{proof}[Proof of the interpolation property (\Cref{prop: general interpolation})]
    We begin by showing that \( g_{\gamma}(X_{\gamma}, \dot{\gamma}) \) is a conserved quantity along any magnetic geodesic \( \gamma \) in the system \( (M, g, \mathrm{d}\alpha) \).\\
Since \( \gamma \) solves \eqref{e:mg}, the time derivative of \( g_{\gamma}(X_{\gamma}, \dot{\gamma}) \) is given by
\begin{equation}\label{eq: derivative of contact angle}
    \frac{\mathrm{d}}{\mathrm{d} t} g_{\gamma}(X_{\gamma}, \dot{\gamma}) = g_{\gamma}\left(\nabla_{\dot{\gamma}} X_{\gamma}, \dot{\gamma} \right) + g_{\gamma}\left(X_{\gamma}, Y_{\gamma}(\dot{\gamma}) \right).
\end{equation}
By using \eqref{eq: Y=2X} and \( Y_{\gamma}(\dot{\gamma}) \perp \dot{\gamma} \), the first term on the right-hand side of~\eqref{eq: derivative of contact angle} vanishes. Using \eqref{eq: Y=2X} again, the second term becomes
\[
2 \cdot g_{\gamma}(X_{\gamma}, \nabla_{\dot{\gamma}} X) = \frac{\mathrm{d}}{\mathrm{d}t} \, g(X_{\gamma}, X_{\gamma}) = \frac{\mathrm{d}}{\mathrm{d}t} \lvert X_{\gamma} \rvert_g^2,
\]
which vanishes because \( \lvert X_{\gamma} \rvert_g \) is constant. This follows from condition \ref{it:prop hyp}, which is by \cite[Lemma 2.2]{ABM} equivalent to the fact that the norm \( \lvert X_{\gamma} \rvert_g \) of the metric dual \( X \) of \( \alpha \) is constant along magnetic geodesics \( \gamma \).
\\
So if $\gc$ is an magnetic geodesic in $(M,g,\d\a)$ with initial values $(\gc(0),\dgc(0))\in \xi$ by \eqref{eq: metric dual is g-orthogonal to xi} and the fact that $g_{\gamma}(X_{\gamma}, \dot{\gamma})$ is an integral of motion the velocity of the magnetic geodesic is horizontal i.e. $\dgc\in \xi_{\gc}$. 
By using this, we can conclude from the fact that $\gamma$ is a minimizer of 
\[
	S_L(\gamma)= \int_0^T \frac{1}{2}g_{\gc(t)}(\dgc(t),\dgc(t)) - \alpha_{\gc(t)}(\dgc(t)) \, \d t
\]
that $\gc$ is also a minimizer of 
\[
	S(\gamma)= \int_0^T \frac{1}{2}g_{\gc(t)}(\dgc(t),\dgc(t)) \, \d t
\]
among all smooth curves such that $\dgc \in \xi := \ker \alpha$. Thus, $\gamma$ is a subriemannian geodesic in $(M, \ker \alpha)$; we refer to~\cite{Montgomereysubriembook} for more background on subriemannian geometry. 

It remains to show that if \( \gamma \) is a magnetic geodesic in \( (M, g, \d\alpha) \) with initial conditions \( (\gamma(0), \dot{\gamma}(0)) \) such that \( \dot{\gamma}(0) = r \cdot X_{\gamma(0)} \) for some \( r \in \mathbb{R} \), then \( \gamma \) is a flow line of \( X \). For simplicity, we assume \( r = 1 \); the general case follows by scaling.\\
To this end, we define the angle \( \theta(t) \) between \( \dot{\gamma}(t) \) and \( X_{\gamma(t)} \) via the relation
\begin{equation}\label{eq: def angle veleocity and X}
    g_{\gamma(t)}(X_{\gamma(t)}, \dot{\gamma}(t)) = \cos(\theta(t)) \cdot \lvert \dot{\gamma}(t) \rvert_g \cdot \lvert X_{\gamma(t)} \rvert_g.
\end{equation}
Note that \( \lvert \dot{\gamma}(t) \rvert_g \) is conserved along the magnetic flow, and similarly, \( \lvert X_{\gamma(t)} \rvert_g \) is constant in time. \begin{comment}
    The latter follows from the identity
\begin{equation}\label{eq: norm of dual of X is constant along magnetic geodesics}
    \frac{\d}{\d t} g_{\gamma}(X_{\gamma}, X_{\gamma}) = g_{\gamma}\left( \left.\nabla_X (2X) \right|_{\gamma}, X_{\gamma} \right) = g_{\gamma}(Y_{\gamma}(\dot{\gamma}(t)), X_{\gamma}),
\end{equation}
where we have used \eqref{eq: Y=2X}. The right-hand side vanishes by the orthogonality condition in \eqref{eq: metric dual is orthogonal to Lorentz force}.
\end{comment} 
Since two of the three factors in \eqref{eq: def angle veleocity and X} are conserved, it follows that \( \cos(\theta(t)) \) is also conserved. From the initial condition \( \dot{\gamma}(0) = X_{\gamma(0)} \), we have \( \theta(0) = 0 \), hence \( \cos(\theta(t)) = 1 \) for all \( t \). This implies
\[
    \dot{\gamma}(t) = X_{\gamma(t)} \quad \text{for all } t \in \mathbb{R},
\]
which completes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%
\subsection{Applications of the interpolation property}

The aim of this subsection is to illustrate \Cref{prop: general interpolation}.
First, we show that in the three-dimensional setting the magnetic geodesic flows
considered therein are totally integrable. Next, we present examples to which
\Cref{prop: general interpolation} applies, focusing on \(K\)-contact manifolds.
Finally, we show that the setting of \Cref{prop: general interpolation} naturally
gives rise to magnetic billiard tables that interpolate between sub-Riemannian
billiards and billiards induced by the Reeb flow.

\paragraph{\textbf{Totally integrable magnetic systems.}}
We begin with an application of the interpolation property from
\Cref{prop: general interpolation} in dimension three, which is of independent
interest.

\begin{cor}\label{cor: total integrability in dim 3}
Let \( g \) be a Riemannian metric and \( \alpha \) a contact one-form on a closed
three-dimensional manifold \( M^3 \), such that \( \alpha \) is Killing with
respect to \( g \), so that condition~\ref{it:prop hyp} holds. Then the magnetic
geodesic flow \( \varPhi^t_{g, \mathrm{d}\alpha} \) of the system
\( (M^3, g, \mathrm{d}\alpha) \) is totally integrable.
\end{cor}

\begin{proof}
Let \( \gamma \) be a magnetic geodesic in \( (M^3, g, \mathrm{d}\alpha) \). Then the
kinetic energy
\[
E = \tfrac{1}{2} \lvert \dot{\gamma} \rvert^2
\]
the angle function \( g_{\gamma}(X_{\gamma}, \dot{\gamma}) \), and the squared norm
\( g_{\gamma}(X_{\gamma}, X_{\gamma}) \) are conserved quantities by
\eqref{eq: derivative of contact angle} and condition~\ref{it:th hyp}. These give
rise to three independent, Poisson-commuting Hamiltonians on \( TM \):
\[
H_1 := E, \qquad
H_2 : TM \to \mathbb{R}, \quad (p,v) \mapsto g_p(X_p, v),
\]
and
\[
H_3 : TM \to \mathbb{R}, \quad (p,v) \mapsto g_p(X_p, X_p).
\]
This implies that the magnetic geodesic flow
\( \varPhi^t_{g, \mathrm{d}\alpha} \) is totally integrable.\todolevin{Add computation that Hamiltonians are poisson commuting to the proof $\rightarrow$ Levin}
\end{proof}

\paragraph{\textbf{Examples: \(K\)-contact manifolds.}}
Next, we illustrate \Cref{prop: general interpolation} on so-called
\(K\)-contact manifolds. We refer to \cite{ABM} and the references therein for
further examples to which this proposition applies, as these provide natural
examples of Killing systems. We then obtain the following result.

\begin{cor}
Let \( (g, \alpha) \) be a \(K\)-contact structure on a manifold \( M \). Then the
magnetic geodesic flow of \( (M, g, \mathrm{d}\alpha) \) interpolates between the
sub-Riemannian geodesic flow on \( (M, \xi := \ker \alpha) \) and the Reeb flow of
\( (M, \alpha) \).
\end{cor}

\todolina{\textbf{Magnetic billiard tables} is missing here, right?}
\todolevin{I can add that if you like :) }

==> Sections/Killing_Magnetic_Systems.tex <==
We recall the definition of a Killing magnetic system introduced in \cite{ABM}.
\begin{defn}
\label{defn: Killing}
An exact magnetic system $(M,g ,\d \alpha)$ on a closed manifold $M$ is called Killing if the $g$-dual $X$ of $\alpha$ is a Killing vector field (i.e., the flow $\Phi_X^t$ of $X$ acts by isometries on $M \,$.) We say that $\alpha$ is Killing for the metric $g$, and that the magnetic Lagrangian $L$ is Killing as well.
\end{defn}

\noindent The following proposition is a straightforward corollary of results in \cite{ABM} and \cite{DMS25Contact}, and shows that the conclusions in~\cite{DMS25Contact} can be applied to magnetic Killing systems.
\begin{prop}
\label{t: main theorem}
Let \((M, g, \mathrm{d}\alpha)\) be a Killing magnetic system. Denote by \(X\) the $g$-dual of \(\alpha \,\). Let $\gamma : [0,T] \rightarrow M $ be a non-constant integral curve of $X$ such that, for all $t\in [0,T], \ \dot\gamma (t) \in\ker(\d \alpha_{\gamma (t)}) \,$.\\
The energy $\kappa$ of $\gamma \,$ is given  by:
$$
\kappa := E(\gamma) = \frac{1}{2} \, |\dot \gamma|^2 = \frac{1}{2} \, |X_\gamma|^2  = \frac{1}{2} \, |\alpha_\gamma|^2  > 0
$$ \lina{that doesn't have to be here}

\lina{I'll get back to it}

\begin{enumerate}[label=(\alph*), resume]
    \item\label{it: Killing main thm - geodesics and magnetic geodesics} 
    All constant reparametrizations $\gamma_r := \gamma(r \,\cdot\,) \comma r \in \IR \,$, are both geodesics of $(M,g)$ and magnetic geodesics of $(M, g, \d \alpha) \,$. The energy of $\gamma_r$ is $E(\gamma_r) = r^2 \, \kappa \,$.
    \item\label{it: Killing main thm - negative action} The action of $\gamma_r$ is
    \begin{align*}
        S_{L + r^2 \kappa}(\gamma_r) = \int_0^T \left( L(\gamma,\dot\gamma) + r^2 \kappa \right) \,\d t = 2 \,r(r -1) \, \kappa \, T
    \end{align*}
    and in particular is negative whenever $0 < r < 1 \,$.
\end{enumerate}
Now suppose additionally that $\gamma : \IR / T \IZ \rightarrow M$ is a contractible loop.
\begin{enumerate}[label=(\alph*), resume]
    \item\label{it: Killing main thm - bound lowest Mane value}
    Then the lowest Ma\~ne critical value can be estimated below by $\kappa \leq c_u(M, g , \d \alpha) \,$.
    \item\label{it: Killing main thm - strong geodesic type} If $\gamma$ has maximal energy $\kappa = \frac{1}{2} \, \lVert \alpha \rVert_\infty \,$, then
    \begin{align*}
        c_u(M,g ,\d \alpha) = \frac{1}{2} \, \lVert \alpha \rVert_\infty \,\, .
    \end{align*}
   If also $\gamma$ is a coorientable loop in $M$, then the system $(M,g,\d \alpha)$ is of strong geodesic type in the sense of \cite{DMS25Contact}.
\end{enumerate}
\todolevin{I would put here only contributions that are not already contained in \cite[§2.2]{ABM}}

\end{prop}


For the next corollaries let $(M,g, \d \alpha)$ always be a Killing magnetic system and let $X$ be the $g$-dual of $\alpha \,$.

\begin{cor}
\label{cor: Killing negative action}
Given any energy level $\kappa > 0 \,$, there are at least as many closed magnetic geodesics of energy $\kappa$ and negative action as there are closed integral curves of $X$ that are tangent to $\ker(\d \alpha) $ and of energy $> \kappa \,$.
\end{cor}

It is well known to experts that conclusion~\ref{it: Killing main thm - negative action} in Theorem~\ref{t: main theorem}, together with \cite[Prop.~2.4]{ConMacPat2004}, yields the following corollary, i.e. provides a negative answer to \Cref{q:Abbond} for the class of spaces considered above, (since \(e_0(M,g,\d\a) = 0\) while \(c_u(M,g,\d\a) \neq 0\)). The details can be found in~\cite[Appendix A]{DMS25Contact}.

\begin{cor}
\label{cor: Killing not contact type} \,
\begin{enumerate}[label=(\alph*)]
    \item\label{it: Killing corollary not contact type < kappa_0} Suppose that $X$ has a closed, contractible integral curve $\gamma$ of energy $\kappa_0 > 0$ that is tangent to $\ker(\d \alpha) \,  $. Then for every level of the energy $\kappa \in (0, \kappa_0)$ the energy hypersurface $\Sigma_\kappa$ is not of contact type.
    \item In particular, if $\gamma$ in Part \ref{it: Killing corollary not contact type < kappa_0} has maximal energy $\kappa = \frac{1}{2} \, \lVert \alpha \rVert_\infty^2 \,$, then every energy hypersurface $\Sigma_\kappa$ for $\kappa \in (0, c_u(M,g,\d\alpha))$ is not of contact type.
\end{enumerate}
\end{cor}

\todolevin{I would kick out both Cor. Thats already known. I would add at beginn, definitions of Killing, and strong geodesic type. Then point out consequences. }





==> Sections/Magnetic_Geodesic_Equation.tex <==
\noindent Let $(M,g ,\sigma)$ be a magnetic system and $\Sigma \subseteq M$ be a hypersurface. Let $i : \Sigma \hookrightarrow M$ denote the inclusion and define
\[ \widetilde{g} := i^* g \quad \text{ and } \quad \widetilde{\sigma} := i^*\sigma \,\, .
\]
We will be interested in magnetic geodesics of the magnetic system $(\Sigma, \widetilde{g} , \widetilde{\sigma}) \,$.
\\
\todolevin{Here we need to motivate, why we are interested in that.}
\todotom{Maybe we could motivate this in the introduction?}
\noindent Because every hypersurface is locally the regular level set of a smooth function $f : U \rightarrow \IR \,$, with $U\subseteq M$ open, and moreover being a magnetic geodesic is a local condition, we may assume without loss of generality that $\Sigma$ is a regular level set.
\\

\noindent So let $f : M \rightarrow \IR$ be smooth with regular value $c \in \IR$ and suppose that $\Sigma = f^{-1}(c) \,$.
\\

\noindent We write $\nabla$ both for the $g$-gradient of a function on $M$ and for the Levi-Civita connection of $g$ respectively $\widetilde{\nabla}$ for the gradient of a function on $\Sigma$ and the Levi-Civita connection of $\widetilde{g} \,$. Similarly, let $Y : TM \rightarrow TM$ denote the Lorentz-force of $(M,g, \sigma)$ and $\widetilde{Y} : T \Sigma \rightarrow T\Sigma$ the Lorentz-force of $(\widetilde{M}, \widetilde{g} , \widetilde{\sigma}) \,$.
Moreover, for every $x \in \Sigma$ we let
\[
P_x : T_x M \rightarrow T_x \Sigma
\]
be the $g_x$-orthogonal projection. Then the orthogonal projection to the complement is given by
\begin{equation}
\label{eq: magnetic geodesic eq - projection complement}
(\mathbbm{1} - P_x) (v) = \frac{g_x(v \comma \nabla f(x))}{|\nabla f(x)|^2} \, \nabla f(x) \,\, .
\end{equation}
(Here $|\,\cdot\,|$ denotes the norm induced by $g_x \,$.)
\\
Write $\mathrm{II}$ for the second fundamental form of $\Sigma \subseteq M \,$. It is well-known that for any curve $\gamma : I \rightarrow \Sigma$ it holds $\nabla_{\dot \gamma} \dot \gamma = \widetilde{\nabla}_{\dot \gamma} \dot \gamma + \mathrm{II}(\dot\gamma, \dot\gamma)$ and in particular
\begin{equation}
\label{eq: magnetic geodesic eq - projection nabla}
    P_{\gamma(t)} (\nabla_{\dot \gamma(t)} \dot \gamma) =  \widetilde{\nabla}_{\dot \gamma(t)} \dot \gamma \,\, .
\end{equation}
Moreover, one readily verifies that the Lorentz forces are related by 
\begin{equation}
\label{eq: magnetic geodesic eq - projection Y}
\widetilde{Y}_x = P_x \circ Y_x |_{T_x \Sigma} \,\, .
\end{equation}

\begin{prop}[Magnetic Geodesic Equation]
\label{prop: magnetic geodesic eq}
Suppose $\Sigma = f^{-1}(c)$ is a regular level set. Let $\gamma : I \rightarrow \Sigma $ be a smooth curve. Then $\gamma$ is a magnetic geodesic of $(\Sigma, \widetilde{g} , \widetilde{\sigma})$ if and only if
\begin{equation}
\label{eq: magnetic geodesic eq}
\nabla_{\dot \gamma} \dot \gamma = Y_\gamma(\dot \gamma) + \frac{g_\gamma(\dot \gamma \comma Y_\gamma(\nabla f (\gamma)) - \nabla_{\dot \gamma} \nabla f )}{|\nabla f(\gamma)|^2} \, \nabla f(\gamma) \,\, .
\end{equation}
\end{prop}
\todolevin{Same applies here, why as a reader should I care about \Cref{prop: magnetic geodesic eq}. What's an use case of this formula?}
\todotom{
In Euclidean space it gives the general second order ODE that magnetic geodesics on hypersurfaces have to satisfy. Given any hypersurface, one "just" has to solve this ODE to determine all magnetic geodesics. See Corollary \ref{cor: magnetic geodesic eq - hypersurface in Euclidean space} below. On an arbitrary manifold, the second order ODE can be written in terms of the covariant derivative. (Working out the Christoffel symbols then again gives a second order ODE in local coordinates.)
}
\todolevin{The main use case that I see so far are numerical simulations. saying that I would be happy if someone prove me wrong.; ) }
\begin{proof}
    Combining \eqref{eq: magnetic geodesic eq - projection complement} with \eqref{eq: magnetic geodesic eq - projection Y} above immediately yields
    \begin{align}
        \widetilde{Y}_\gamma(\dot \gamma) &= Y_\gamma(\dot \gamma) - \frac{g_\gamma(Y_\gamma(\dot \gamma) \comma \nabla f (\gamma))}{|\nabla f (\gamma)|^2} \, \nabla f(\gamma) \notag\\
        &= Y_\gamma(\dot \gamma) + \frac{g_\gamma(\dot \gamma \comma Y_\gamma(\nabla f (\gamma)))}{|\nabla f (\gamma)|^2} \, \nabla f(\gamma)
        \,\, ,
        \label{eq: magnetic geodesic eq - Ytilde gammadot}
    \end{align}
    where the second equation followed from skew-symmetry of $Y \,$.
    \\
    Similarly, \eqref{eq: magnetic geodesic eq - projection complement} and \eqref{eq: magnetic geodesic eq - projection nabla}, give
    \begin{align}
       \widetilde{\nabla}_{\dot\gamma}(\dot \gamma) &= \nabla_{\dot\gamma}\dot \gamma - \frac{g_\gamma(\nabla_{\dot \gamma}\dot \gamma \comma \nabla f (\gamma))}{|\nabla f (\gamma)|^2} \, \nabla f(\gamma) \notag\\
       &= \nabla_{\dot\gamma}\dot \gamma + \frac{g_\gamma(\dot \gamma \comma \nabla_{\dot \gamma} \nabla f)}{|\nabla f (\gamma)|^2} \, \nabla f(\gamma) \,\, ,
       \label{eq: magnetic geodesic eq - nablatilde gammadot}
    \end{align}
    where the second equation followed from compatibility of $\nabla$ with $g$ and 
    \[
    \frac{\d}{\d t} \, g_\gamma(\dot \gamma \comma \nabla f(\gamma)) =  \frac{\d}{\d t} \big(\underbrace{\d f_\gamma(\dot \gamma)}_{= 0} \big) = 0 \,\, .
    \]
    Subtracting \eqref{eq: magnetic geodesic eq - Ytilde gammadot} from \eqref{eq: magnetic geodesic eq - nablatilde gammadot}, we see that
    \begin{align*}
       \widetilde{\nabla}_{\dot\gamma}(\dot \gamma) -  \widetilde{Y}_\gamma(\dot \gamma) = 
       \nabla_{\dot \gamma} \dot\gamma - Y_\gamma(\dot \gamma) - \frac{g_\gamma(\dot \gamma \comma  Y_\gamma(\nabla f(\gamma)) - \nabla_{\dot \gamma} \nabla f)}{|\nabla f(\gamma)|^2} \, \nabla f(\gamma) \,\, .
    \end{align*}
    Finally, $\gamma$ is a magnetic geodesic of $(\Sigma, \widetilde{g}, \widetilde{\sigma})$ iff the left-hand side in the above equation vanishes and the latter is equivalent to \eqref{eq: magnetic geodesic eq}.
\end{proof}

Notice that \eqref{eq: magnetic geodesic eq} is a second-order differential equation formulated entirely in the ambient manifold $M \,$. Its right-hand side contains the covariant Hessian $\nabla \nabla f$ of $f$ in direction $\dot\gamma \,$.

\subsection{Hypersurfaces in Euclidean Space}
\label{subsection: magnetic geodesic eq - Euclidean space}

In the special case where $\Sigma = f^{-1}(c)$ is a regular level set in the Euclidean magnetic system 
\[
(M=\IR^{2n} = \IC^{n} \comma g= g_{\mathrm{euc}} = \langle \,\cdot\comma\cdot\, \rangle_{\IR} \comma \sigma = \omegacan) \,\, ,
\]
where we abbreviate the Euclidean inner product by $\langle \,\cdot\comma \cdot\, \rangle_{\IR}$ to not confuse it with the standard Hermitian inner product $\langle\,\cdot\comma \cdot\,\rangle \,$, the Lorentz force $Y$ is just multiplication by the imaginary unit $\i$ and \Cref{prop: magnetic geodesic eq} becomes 
\begin{cor}
\label{cor: magnetic geodesic eq - hypersurface in Euclidean space}
A smooth curve $\gamma : I \rightarrow \Sigma = f^{-1}(c)$ is a magnetic geodesic of the magnetic system
$$
(\Sigma , \widetilde{g} , \widetilde{\sigma}) := (\Sigma \comma g_{\mathrm{euc}}|_{\Sigma} \comma \omegacan|_{\Sigma})
$$ 
if and only if
\begin{equation}
\label{eq: magnetic geodesic eq - hypersurface in Euclidean space}
\ddot \gamma = \i\, \dot\gamma + \frac{\langle \dot \gamma \comma \i \,\nabla f(\gamma) \rangle_{\mathrm{\IR}} - \mathrm{Hess}_\gamma(f) \, [\dot\gamma, \dot\gamma]}{|\nabla f (\gamma)|^2} \, \nabla f(\gamma) \,\, .
\end{equation}
\end{cor}

The following lemma will play a role in the application of \Cref{cor: magnetic geodesic eq - hypersurface in Euclidean space} to complex ellipsoids.

\begin{lem}
\label{lem: magnetic geodesic eq - < gammadot , i nabla f >}
For a magnetic geodesic $\gamma: I \rightarrow \Sigma $ of $(\Sigma , \widetilde{g} , \widetilde{\sigma})$ we have
\[
\frac{\d}{\d t} \, \langle \dot\gamma \comma \i \, \nabla f (\gamma) \rangle_{\IR} = - \mathrm{Hess}_\gamma(f) \, [\dot\gamma \comma \i \,\dot\gamma] \,\, .
\]
\end{lem}

\begin{proof}
We start by computing the derivative
    \begin{align*}
        \frac{\d}{\d t} \Rproduct{\dot\g}{\i \, \nabla f (\gamma)} &= \Rproduct{\ddot\g}{\i \, \nabla f(\gamma)} + \Rproduct{\dot\g}{\i \cdot \Hess_\gamma(f) \cdot \dot\g} \\
        &= \Rproduct{\ddot\g}{\i \, \nabla f(\gamma)} - \Rproduct{\i \cdot \dot\g}{\Hess_{\gamma} (f) \cdot \dot\g} \,\, .
    \end{align*}
    The lemma follows if we show that the first summand on the right-hand side vanishes.
    As above, we write $P_z : \IR^{2n} \rightarrow T_z \Sigma$ for the orthogonal projection. Because $\i \, \nabla f (z) $ lies in $\mathrm{span}\{\nabla f(z)\}^{\perp} = T_z \Sigma \,$, we have
\begin{align}
\label{eq: magnetic geodesic eq - (v, i nabla f)}
    \Rproduct{v}{\i \, \nabla f (z)} = \Rproduct{P_{z} \, v}{\i \, \nabla f (z)} \qquad \forall \, v \in \IR^{2n} \,\, .
\end{align}
Taking into account that $ P_\gamma(\ddot\g) = P_\gamma ( \i\, \cdot \dot\g) $ by \eqref{eq: magnetic geodesic eq - projection nabla} and \eqref{eq: magnetic geodesic eq - projection Y} and since $\g$ is a magnetic geodesic of $(\Sigma , \widetilde{g} , \widetilde{\sigma} ) \,$, we obtain
\begin{align*}
    \Rproduct{\ddot\g}{\i \, \nabla f(\gamma)} &\overset{\text{\eqref{eq: magnetic geodesic eq - (v, i nabla f)}}}{=} \Rproduct{P_\g ( \, \ddot\g ) }{\i \, \nabla f (\g)} =  \Rproduct{P_\g (\i \cdot \dot\gamma) }{\i \, \nabla f (\g)} \overset{\text{\eqref{eq: magnetic geodesic eq - (v, i nabla f)}}}{=}  \Rproduct{\i \cdot \dot\g}{ \i \, \nabla f (\g)} \\
    &\hspace*{1.5mm}= \Rproduct{\nabla f (\g)}{\dot\g}  = 0 \,\, .
\end{align*}
The last equation holds since $\gamma$ maps to the level set $\Sigma = f^{-1}(c) \,$.
\end{proof}

\subsection{Application to Ellipsoids}
\label{subsection: magnetic geodesic equation - Application to Ellipsoids}

We continue with the setting of \Cref{section: Illustration on Ellipsoids} and, for the matrix $A=\mathrm{diag}(a_1,\ldots , a_n)$ associated to the increasing sequence $0 < a_1 \leq \ldots \leq a_{n} \,$, consider the ellipsoid $E(A)$  inside the Euclidean magnetic system
\[
(M= \IC^{n} \comma g = g_{\mathrm{euc}} = \mathrm{Re} \, \langle \,\cdot\comma \cdot\,\rangle \comma \sigma = \omegacan ) \,\, .
\]
We note that the restriction of this magnetic system to $E(A)$ is the system $(E_A , g , \d \alpha)$ which we described in \Cref{section: Illustration on Ellipsoids}. Let us use \Cref{cor: magnetic geodesic eq - hypersurface in Euclidean space} to determine the ordinary differential equation that magnetic geodesics on $E(A)$ have to satisfy.
\\

\noindent The ellipsoid $E(A)$ is the level set (for regular value $1$) of the function $f : \IC^{n} \rightarrow \IR$ defined by 
$$
f(z) = f(z_1, \ldots , z_{n}) = \sum_{j=1}^{n} \frac{|z_j|^2}{a_j} \,\, .
$$ Its gradient 
$$
\nabla f (z) = 2 \, A^{-1} \, z = \left(\frac{2}{a_1} z_1 \comma \ldots \comma \frac{2}{a_{n}} z_{n} \right) \in \IC^{n+1}
$$ 
has squared norm $\sum_{j=1}^{n} \frac{4}{a_j^2} |z_j|^2 \,$. The Hessian of $f$ computes to 
$$
\Hess_{z}(f) = 2\,A^{-1} = 2 \, \mathrm{diag}(a_1^{-1}, \ldots , a_{n}^{-1})  \in \mathrm{GL}(n, \IC) \,\, .
$$ 
We conclude with \Cref{cor: magnetic geodesic eq - hypersurface in Euclidean space} that
 a curve $\gamma : I \rightarrow E(A)$ is a magnetic geodesic on the ellipsoid if and only if
\begin{align*}
    \ddot \g = \i \cdot \dot \g + \frac{1}{\sum_{j=1}^n \frac{4}{a_j^2} |\gamma_j|^2} \left( 
 \Rproduct{\dot\g}{\i \, \nabla f(\gamma)} - 2 \sum_{j=1}^n \frac{|\dot\g_j|^2}{a_j}
 \right) \,\, 2 \, A^{-1} \,\gamma \,\, .
\end{align*}
We note that, for a magnetic geodesic $\gamma \,$, the term $\Rproduct{\dot\gamma}{\i \, \nabla f (\gamma)}$ is an integral of motion, as by Lemma \ref{lem: magnetic geodesic eq - < gammadot , i nabla f >} we have
\[
\frac{\d}{\d t} \, \langle \dot\gamma \comma \i \, \nabla f (\gamma) \rangle_{\IR} = - \mathrm{Hess}_\gamma(f) \, [\dot\gamma \comma \i \cdot \dot\gamma] = \sum_{j=1}^{n} \frac{2}{a_j} \, \Rproduct{\dot\gamma}{\i \cdot \dot\gamma} = 0 \,\, .
\]
(In the special case of the sphere this has already been established in \cite{ABM}. The conserved quantity is called the \textit{contact angle} therein.) We summarize the above discussion in the following corollary.

\begin{cor}
\label{cor: magnetic geodesic eq - ellipsoids}
\begin{enumerate}[label=(\alph*)]
    \item\label{it: magnetic geodesic eq - ellipsoids} For a magnetic geodesic $\gamma : I \rightarrow E(A)$ the quantity 
    $$
    C_\gamma := \frac{1}{2} \,\Rproduct{\dot\gamma}{\i \,\nabla f(\gamma)}
    $$ 
    is conserved and
     \begin{equation}\label{eq: magnetic geodesic eq - ellipsoids}
    \ddot\gamma = \i \cdot \dot\gamma + \frac{C_\gamma - \sum_{j=1}^{n} \frac{1}{a_j} \, |\dot\gamma_j|^2 }{\sum_{j=1}^{n}  \frac{1}{a_j^2} \, |\gamma_j|^2} \, \left( \frac{\gamma_1}{a_1} , \ldots , \frac{\gamma_{n}}{a_{n}} \right) \,\, .
    \end{equation}
    Moreover, letting $\kappa :=|\dot\gamma|$ denote the (constant) velocity of $\gamma \,$, it holds
    \[
    |C_\gamma| \leq \kappa \, \inf_I \sqrt{\sum_{j=1}^{n} \frac{1}{a_j^2} \, |\gamma_j|^2}  \,\, .
    \] 
    \item\label{it: magnetic geodesic eq - ellipsoids converse} Conversely, given a curve $\gamma : I \rightarrow E(A)$ that satisfies \eqref{eq: magnetic geodesic eq - ellipsoids} with $C_\gamma := \tfrac{1}{2} \, \Rproduct{v}{\i \, \nabla f(z)} \,$, where $z := \gamma(0)$ and $v:= \dot\gamma(0) \,$. Then $\gamma$ is a magnetic geodesic on the ellipsoid.
\end{enumerate}
\end{cor}
\todolevin{I would ike to understand that better. Because what is the benefit of that compared of doing the following: using the magnetomorphism in \Cref{section: Illustration on Ellipsoids} and combining it with an argument along the lines in \cite{BM24}, I get for each coordinate axis an intregral of motion. Consequentely we get a) as special case.}
\todotom{
You can probably equally well apply \cite{BM24} to derive that result. It just illustrates Proposition \ref{prop: magnetic geodesic eq} and Corollary \ref{cor: magnetic geodesic eq - hypersurface in Euclidean space} with an example where one can still explicitly compute stuff. Corollary \ref{cor: magnetic geodesic eq - hypersurface in Euclidean space} is interesting, because it gives the general ODE for magnetic geodesics on arbitrary hypersurfaces. The ellipsoid just illustrates it. Plus, the symmetry of the ellipsoid allows for a conserved quantity, namely $\langle \dot\g, \i  \nabla f(\g) \rangle$, so that the ODE gets easier to solve.
}
\todolevin{We are not able to solve the ODE right? For which f is  $\langle \dot\g, \i  \nabla f(\g) \rangle$ a integral of motion? 
In case of an ellipsoid we get by the other approach that this intergral is an linear combination of $(n+1)$ independent poisson commuting intergrals of motion. }
\todotom{$\langle \dot\g, \i  \nabla f(\g) \rangle$ is an integral of motion iff $\mathrm{Hess}_\gamma(f) [\dot\gamma,\i \,\dot \gamma]$ vanishes identically, by Lemma \ref{lem: magnetic geodesic eq - < gammadot , i nabla f >}. In general we cannot solve the ODE \eqref{eq: magnetic geodesic eq - ellipsoids}.} 
\begin{proof}
    Part \ref{it: magnetic geodesic eq - ellipsoids} was proven above. The estimate for $|C_\gamma|$ follows with Cauchy-Schwarz.\\
    For Part \ref{it: magnetic geodesic eq - ellipsoids converse}, given $z = \gamma(0)$ and $v := \dot\gamma(0) \,$, consider the unique magnetic geodesic $\gamma_{v}$ with initial conditions $\gamma_v(0) = z$ and $\dot\gamma_v(0)= v \,$. Then both $\gamma$ and $\gamma_v$ satisfy \eqref{eq: magnetic geodesic eq - ellipsoids} with $C_\gamma $ and have the same initial conditions. From uniqueness of solutions to ordinary differential equations, we infer $\gamma = \gamma_v \,$.
\end{proof}

In the case of the sphere $\SS^{2n-1}_r$ of radius $r \,$, that is $a_1 = \ldots = a_{n} = r \,$, the above differential equation \eqref{eq: magnetic geodesic eq - ellipsoids} has a particularly convenient form: For a magnetic geodesic $\gamma : I \rightarrow \SS^{2n-1}_r$ we have $\sum_j |\gamma_j|^2 = |\gamma|^2 = r^2$ and hence
\[
\ddot \gamma = \i \cdot \dot\gamma + \left(C_\gamma - \frac{1}{r^2} \, |\dot\gamma|^2 \right) \, \gamma \qquad \text{ where } C_\gamma \in \left[ - \frac{|\dot\gamma|}{r}  \comma \frac{ |\dot\gamma|}{r}\right] \,\, .
\] 
In the case of a unit speed magnetic geodesic $\gamma$ we can introduce $\psi_\gamma \in [0,\pi]$ via $\cos(\psi_\gamma) = r \, C_\gamma $ and the above differential equation becomes
\[
0 = \ddot \gamma - \i \cdot \dot \gamma  + \frac{1}{r^2} \left( 1 - r \, \cos(\psi_\gamma) \right) \, \gamma \,\, .
\]
For $r=1$ this recovers \cite[Eq. (3.2)]{ABM}. The above formula is a linear ODE and can be readily solved.





==> Sections/Magnetomorphisms.tex <==

\todolevin{Again the motivation and overview is missing. }
For a magnetic system $(M,g , \sigma)$ the \textit{group of magnetomorphisms} was defined in \cite{ABM} as
\begin{align*}
    \mathrm{Mag}(M, g , \sigma) := \set{\psi \in \mathrm{Diff}(M)}{\psi^*g = g \text{ and } \psi^* \sigma = \sigma } \quad .
\end{align*}
We compute the group of magnetomorphisms for closed strictly convex hypersurfaces in $\IR^{2n} \,$.

In the following, for a matrix $A \in \IR^{2n \times 2n}$ and a vector $b \in \IR^{2n}$ we write $F_{A,b} : \IR^{2n} \rightarrow \IR^{2n}$ for the affine linear transformation 
$$
F_{A,b}(x) = A x + b \,\, .
$$
A closed (i.~e. compact and without boundary) and connected hypersurface $\Sigma \subseteq \IR^{2n}$ is \textit{strictly convex} if it bounds a strictly convex body.

\begin{prop}
\label{prop: magnetomorphism group}
Let $\Sigma \subseteq \IR^{2n} \comma n \geq 2 \,$, be a strictly convex hypersurface and denote by $i : \Sigma \hookrightarrow \IR^{2n}$ the inclusion. Then the map
\begin{align*}
    \mathrm{G}_\Sigma := \set{F_{U,b}}{ U \in \mathrm{U}(n ) \comma b \in \IR^{2n} \text{ with } F_{U,b}(\Sigma) = \Sigma } &\rightarrow \mathrm{Mag}(\Sigma , \, i^*g_{\mathrm{euc}} , \, i^* \omegacan) \\
    F \mapsto F|_\Sigma
\end{align*}
is a group isomorphism.
\end{prop}

The next lemma prepares the proof of the proposition. Its proof is elementary.

\begin{lem}
\label{lem: magnetomorphism group - F_(A,b) = id}
For $A \in \O(2n)$ and $b \in \IR^{2n}$ and any closed hypersurface $\Sigma \subseteq \IR^{2n}$ it holds: If $F_{A,b} |_\Sigma = \id_{\Sigma} \,$, then $A = \mathbbm{1}$ and $b= 0$.
\end{lem}

\begin{proof}
    The proof relies on the fact that $\Sigma$ is not contained in a proper affine linear subspace. If $b \not= 0 \,$, then $2  \Rproduct{Ax}{b} + |b|^2=0$ for $x \in \Sigma$ since $|Ax + b|^2 = |x|^2 = |Ax|^2$ by assumption. Thus $A \cdot \Sigma $ is contained in the proper affine linear subspace given by the equation $2 \Rproduct{y}{b} + |b|^2=0 \,$, contradiction. Hence $b= 0$ and so $F_{A,b}=F_{A,0}$ is a linear isometry with $\Sigma \subseteq \mathrm{Eig}(1,A) \,$. It follows that the eigenspace of $A$ for eigenvalue $1$ is the whole $\IR^{2n} \,$.
\end{proof}

\begin{proof}[Proof of \Cref{prop: magnetomorphism group}]
    Observe that $G_\Sigma$ is (with the composition of maps as operation) indeed a group. Recall that the two-out-of-three property in particular says that
    \begin{equation}
    \label{eq: magnetomorphism group - 2 out of 3}
    \mathrm{U}(n) = \mathrm{O}(2n) \cap \mathrm{Sp}(2n) \,\, .
    \end{equation}
    So the map from $G_\Sigma$ to the magnetomorphism group is a well-defined group homomorphism. Lemma \ref{lem: magnetomorphism group - F_(A,b) = id} implies that its kernel is trivial. We must show that it is also onto.\\
    To this end, let $\psi : \Sigma \rightarrow \Sigma$ be an arbitrary magnetomorphism of $(\Sigma, i^*g_{\mathrm{euc}} , i^*\omegacan) \,$. It is a fact that every Riemannian isometry of a strictly convex hypersurface in Euclidean space is the restriction of a congruence (that is a Riemannian isometry of the ambient Euclidean space), see \cite[Thm. 2]{Survey_Convex_Hypersurfaces} or \cite[Thm. V]{Sacksteder}. Hence there exist $A \in \O(2n)$ and $b \in \IR^{2n}$ with $\psi = F_{A,b} |_\Sigma^{\Sigma} \,$. It remains to verify that $A \in \Unitary(n) \,$. In view of \eqref{eq: magnetomorphism group - 2 out of 3} it suffices to show that $A$ is a symplectic matrix. Let $v_1, v_2 \in \IR^{2n}$ be arbitrary. Since $\Sigma$ is strictly convex, there exists a point $p \in \Sigma$ with $v_1, v_2 \in T_p \Sigma \,$.\footnote{
    To see this, choose any unit vector $u$ orthogonal to both $v_1$ and $v_2$. Recall that the Gauss map $\Sigma \rightarrow \SS^{2n-1}$ is defined by mapping $q \in \Sigma$ to the outward pointing unit normal vector $\nu_q$ of $\Sigma$ at $q \,$.
    Since $\Sigma$ is a strictly convex hypersurface, its Gauss map is bijective. Now the unique $p \in \Sigma$ with $\nu_p = u$ has the property that $v_1,v_2 \in T_p \Sigma \,$.
    }
    Since $\psi$ is a magnetomorphism, we then have
    \begin{align*}
        \omegacan(v_1 \comma v_2) = (i^* \, \omegacan)_p (v_1 \comma v_2) = (i^* \, \omegacan)_{\psi(p)} (d_p \psi \,\, v_1 \comma d_p \psi \,\, v_2) = \omegacan (A v_1 \comma A v_2 ) \,\, .
    \end{align*}
    Hence $A$ is indeed symplectic. This finishes the proof.
\end{proof}

We finish our considerations by providing a means to determine the affine shift $b$ of a magnetomorphism $F_{U,b} \,$. We first recall the following fact.

\begin{rem}
\label{rem: magnetomorphism group - Jordan-Brouwer separation}
Let $\Sigma \subseteq \IR^{2n}$ be a strictly convex hypersurface. By the Jordan-Brouwer separation theorem $\IR^{2n} - \Sigma$ consists of precisely two connected components, one of which is bounded. We call this the \textit{inside component} and denote it by $B \,$. Notice that the closure $\overline{B}$ is a strictly convex body bounding $\partial \overline{B} =\Sigma$. It is well-known, see \cite[Lemma 2.8]{Inscribed_Ball_Convex_Body}, that every strictly convex body has a unique inscribed ball of maximal radius. The center of this ball is the unique point $x_0 \in B$ with $\mathrm{dist}(x_0, \Sigma) = \sup_{x \in B} \mathrm{dist}(x, \Sigma) \,$.
\end{rem}

For the following lemma let $\Sigma$ be a strictly convex hypersurface with inside component $B$ and let $x_0 \in B$ be the unique point with $\mathrm{dist}(x_0, \Sigma) = \sup_{x \in B} \mathrm{dist}(x, \Sigma) \,$.

\begin{lem}
 \label{lem: magnetomorphism group - determining b}   
 Given $A \in \O(2n)$ and $b \in \IR^{2n}$ with $F_{A,b}(\Sigma) = \Sigma \,$. Then $b = (\mathbbm{1} - A) x_0 \,$. In particular, $b= 0$ if $x_0 = 0 \,$.
\end{lem}

\begin{proof}
    Abbreviate $F := F_{A,b} \,$. Notice that $F(B)$ is bounded by continuity.
    Since the homeomorphism $F : \IR^{2n} - \Sigma \rightarrow \IR^{2n} - \Sigma$ maps connected components to connected components, we infer that $F(B)=B \,$, so that in particular $F(x_0) \in B \,$. Because $F$ is distance preserving, furthermore
    \begin{align*}
        \mathrm{dist}(F(x_0) \comma \Sigma) = \mathrm{dist}(F(x_0) \comma  F(\Sigma)) = \mathrm{dist}(x_0 \comma \Sigma ) = \mathrm{sup}_{x \in B} \,\mathrm{dist}(x,\Sigma) \,\, .
    \end{align*}
    From uniqueness of $x_0$ we conclude that $x_0 = F(x_0 ) = A x_0 + b \,$.
\end{proof}

\begin{cor}
\label{cor: magnetomorphism group - with x_0 = origin}
Let $i : \Sigma \hookrightarrow \IR^{2n} \comma n \geq 2 \,$, be a strictly convex hypersurface for which the inscribed ball of maximal radius is centered at the origin. Then 
\begin{align*}
    \set{U \in \Unitary(n)}{ U \cdot \Sigma = \Sigma} &\rightarrow  \mathrm{Mag}(\Sigma , \, i^*g_{\mathrm{euc}} , \, i^* \omegacan) \\
    U &\mapsto F_{U,0} \,|_\Sigma 
\end{align*}
is a group isomorphism.
\end{cor}

\begin{proof}
    This follows from \Cref{prop: magnetomorphism group} and Lemmata \ref{lem: magnetomorphism group - F_(A,b) = id} and \ref{lem: magnetomorphism group - determining b}.
\end{proof}
\todolevin{That's cool. Thats helpful in order to get integrals of motion.}

\subsection{Application to Ellipsoids}
\label{subsection: magnetomorphism group - Ellipsoids}

As an application, let us compute the group of magnetomorphisms of a complex ellipsoid (introduced in \Cref{section: Illustration on Ellipsoids}). For convenience, we slightly alter the notation for ellipsoids. Given $\mathbf{a}=(\mathbf{a}_1, \ldots , \mathbf{a}_k)$ with $\mathbf{a}_j = (a_j , \ell_j) \in (0, + \infty) \times \IN_{\geq 1}$ such that $a_1 < \ldots < a_k$ and $\sum_{j=1}^k \ell_j = n \,$, we write $E(\mathbf{a})$ for the complex ellipsoid in $\IC^n$ associated to the increasing sequence
\begin{align*}
    \underbrace{a_1 = \ldots = a_1}_{\ell_1\text{-times}} < \underbrace{a_2 = \ldots = a_2}_{ \ell_2\text{-times}} < \ldots < \underbrace{a_k = \ldots = a_k}_{\ell_k \text{-times}} \,\, .
\end{align*}

\begin{prop}
\label{prop: magnetomorphism group - Ellipsoids}
 For $n \geq 2$ the group of magnetomorphisms of $E(\mathbf{a}) $ is isomorphic to
    \begin{align*}
        \Unitary(\ell_1) \times \ldots \times \Unitary(\ell_k) \,\, .
    \end{align*}
    An explicit isomorphism is given by $(U_1 \comma \ldots \comma U_k) \mapsto \mathrm{diag}(U_1, \ldots , U_k) |_{E(\mathbf{a})} \,$.
\end{prop}

\begin{rem}
\label{rem: magnetomorphisms sphere}
    It is proven in \cite[Cor. 1.5]{ABM} that the magnetomorphism group of the sphere $\SS^{2n-1}$ is $\mathrm{U}(n) \,$. The above proposition retrieves this result in the special case $k=1 \,$.
\end{rem}

\Cref{prop: magnetomorphism group - Ellipsoids} follows immediately from \Cref{cor: magnetomorphism group - with x_0 = origin} and the next lemma.

\begin{lem}
\label{lem: magnetomorphism group - U E(a) = E(a)}
Suppose that $U \in \Unitary(n)$ satisfies $U \cdot E(\mathbf{a}) = E(\mathbf{a})$. Then there exist $U_1 \in \Unitary(\ell_1) \comma \ldots \comma U_{k} \in \Unitary(\ell_k)$ such that $U=\mathrm{diag}(U_1, \ldots , U_k) \,$.
\end{lem}

\begin{proof}
    We will show by an induction on $k$, that for every $n \geq 1$, every $\mathbf{a}=(\mathbf{a}_1, \ldots , \mathbf{a}_k) = ((a_1, \ell_1) \comma \ldots \comma (a_k , \ell_k))$ with $a_1 < \ldots < a_k$ and $\sum_{j=1}^k \ell_j = n$ and every $U \in \Unitary(n)$ it holds
    \begin{align*}
        U \cdot E(\mathbf{a}) = E(\mathbf{a}) \,\, \Longrightarrow \,\, \Exists U_1 \in \Unitary (\ell_1), \ldots , U_k \in \Unitary(\ell_k) : \quad U= \mathrm{diag}(U_1, \ldots , U_k) \,\, .
    \end{align*}
    The induction basis $k=1$ holds trivially. Now let $k \geq 2$ be arbitrary and assume the statement for $k-1$ is true. For $n =1$ the statement is void since $\sum_{j=1}^k \ell_j \geq 2 \,$. Now let $n \geq 2$ and $\mathbf{a} = (\mathbf{a}_1, \ldots , \mathbf{a}_k)$ be as above. For $U \in \Unitary(n)$ assume $U \cdot E(\mathbf{a}) = E(\mathbf{a}) \, $. For $\mathbf{z} = (z_1, \ldots , z_n) \in \IC^n$ we also write 
    $$
    \mathbf{z} = (\mathbf{z}_1, \ldots , \mathbf{z}_k) \in \IC^{\ell_1} \times \ldots \times \IC^{\ell_k} \,\, .
    $$
    Since $a_1 < \ldots < a_k $ is strictly increasing, a vector $\mathbf{z} \in E(\mathbf{a})$ maximizes the norm on $E(\mathbf{a})$ if and only if it is of the form $\mathbf{z}=(\mathbf{0}, \ldots , \mathbf{0}, \mathbf{z}_k) \,$. Therefore, since $U$ is norm-preserving, $U$ must map 
    $$
    E(\mathbf{a}) \cap (\{\mathbf{0}\} \times \ldots \times \{ \mathbf{0} \} \times \IC^{\ell_k})
    $$
    to itself. Thus $U \in \Unitary(n)$ is a block matrix of the form
    \begin{align*}
        U = \left( \begin{matrix}
            \widetilde{U} & 0 \\
            B & U_k
        \end{matrix} \right) \in \IC^{n \times n}
    \end{align*}
    for certain matrices $\widetilde{U} \in \IC^{(n - \ell_k) \times (n - \ell_k)} \comma B \in \IC^{\ell_k \times (n - \ell_k)}$ and $U_k \in  \IC^{\ell_k \times  \ell_k} \,$. Since $U$ is a unitary matrix, we conclude that $B=0$ and that both $\widetilde{U}$ and $U_k$ are unitary. Using again that $U \cdot E(\mathbf{a}) = E(\mathbf{a})$, we also have
    \begin{align*}
        \widetilde{U} \cdot E(\mathbf{a}_1, \ldots , \mathbf{a}_{k-1}) = E(\mathbf{a}_1, \ldots , \mathbf{a}_{k-1}) \subseteq \IC^{n - \ell_k} \,\, .
    \end{align*}
    Now apply the induction hypothesis to $\widetilde{U}$, finishing the induction step.
\end{proof}





==> Sections/Totally_Magnetic_Submanifolds.tex <==
The notion of a totally magnetic submanifold was introduced in \cite{ABM}. We recall its definition.
\begin{defn}[Totally magnetic Submanifold]
%\label{defn: totally magnetic submfds}
Let $(M,g,\sigma)$ be a magnetic system. An (embedded) submanifold $N \subseteq M$ is called \textit{totally magnetic} if for all magnetic geodesics $\gamma : I \rightarrow M$ with $\gamma(0) \in N$ and $\dot\gamma(0) \in T_{\gamma(0)} N$ there is an $\e > 0$ for which $\gamma((-\e,\e)) \subseteq N \,$.
\end{defn}

Totally magnetic submanifolds should be understood as totally geodesic submanifolds for which the tangent bundle is invariant under the Lorentz force of the magnetic system $(M,g,\sigma) \,$, as the following characterization specifies.

\begin{thm}[\cite{ABM}, Thm. 1.4]
%\label{t: totally magnetic submfds - characterization totally magnetic from ABM}
Let $(M,g,\sigma)$ be a magnetic system with Lorentz force $Y : TM \rightarrow TM $ and let $N \subseteq M$ be a submanifold. Denote by $i : N \hookrightarrow M$ the inclusion.
The following are equivalent.
\begin{enumerate}[label=(\roman*)]
    \item $N$ is a totally magnetic submanifold of $(M,g,\sigma) \,$.
    \item Every magnetic geodesic $\gamma : I \rightarrow N$ of $(N , i^*g, i^*\sigma)$ is also a magnetic geodesic of $(M,g,\sigma) \,$.
    \item $N$ is a totally geodesic submanifold of $(M,g)$ and $Y_p(T_p N) \subseteq T_p N $ for all $p \in N \,$.
\end{enumerate}
\end{thm}

In the following let $(M,g , \sigma)$ always be a magnetic system.

\begin{rem}
\label{rem: totally magnetic submfds - transitive}
Given submanifolds $\widetilde{N} \subseteq N \subseteq M \,$. Denote by $i : N \hookrightarrow M$ the inclusion. Observe that, if $\widetilde{N}$ is totally magnetic for $(M,g ,\sigma) \,$, then $\widetilde{N}$ is also totally magnetic for $(N, i^*g, i^* \sigma) \,$.
\end{rem}

We state two results about totally magnetic submanifolds that resemble the totally geodesic case.

\begin{prop}
%\label{prop: totally magnetic submfds - fixed point set}
Let $\mathcal{M} \subseteq \mathrm{Mag}(M,g,\sigma)$ be a subset of magnetomorphisms. Then each connected component of the fixed point set
\[
\mathrm{Fix}(\mathcal{M}) = \set{p ´\in M}{F(p) = p \quad \forall \, F \in \mathcal{M}}
\]
is a totally magnetic submanifold of $(M,g,\sigma) \,$.
\end{prop}

\begin{prop}
%\label{prop: totally magnetic submfds - intersections}
Given two totally magnetic submanifolds $N_1, N_2 \subseteq M $ of $(M,g,\sigma) \,$. Then each connected component of $N=N_1 \cap N_2$ is a totally magnetic submanifold of $(M,g,\sigma) $ with tangent space $T_p N_1 \cap T_p N_2$ at $p \in N \,$.
\end{prop}

We prove the preceding propositions in the subsequent subsection.

\subsection{Proofs of Propositions \ref{prop: totally magnetic submfds - fixed point set} and \ref{prop: totally magnetic submfds - intersections}}
\label{subsection: totally magnetic submfds - proofs of fixed point and intersection prop}

We first recall the definition of the Zariski tangent space. Given a subset $\mathcal{M} \subseteq \mathrm{Isom}(M,g)$ of isometries. For $p \in \mathrm{Fix}(\mathcal{M})$ the Zariski tangent space $\mathrm{Z}_p$ at $p$ is defined by
     \begin{equation}
      \mathrm{Z}_p := \set{v \in T_p M}{ \d_p F \cdot v = v \quad \forall \, F \in \mathcal{M}} \subseteq T_p M \,\, .    
     \end{equation}
     It is shown in \cite[Prop. 5.6.5]{Pet} that $\exp_p^M : B_\e(0) \cap \mathrm{Z}_p \rightarrow B_\e(p) \cap N$ is a well-defined slice chart for $\e > 0$ sufficiently small, so that the connected components of $\mathrm{Fix}(\mathcal{M})$ are totally geodesic submanifolds with tangent space at $p$ equal to the Zariski tangent space $\mathrm{Z}_p \,$.



\begin{proof}[Proof of \Cref{prop: totally magnetic submfds - fixed point set}]
    Because $\mathcal{M} \subseteq \mathrm{Mag}(M,g,\sigma)$ is in particular a subset of isometries of $(M,g) \,$, the above discussion already shows that the connected components of $\mathrm{Fix}(\mathcal{M})$ are totally geodesic submanifolds of $(M,g)$, having the Zariski tangent spaces as tangent spaces. By \Cref{t: totally magnetic submfds - characterization totally magnetic from ABM}, to finish the proof, it suffices to show that for every $p \in \mathrm{Fix}(\mathcal{M})$ the Lorentz force $Y_p : T_p M \rightarrow T_p M$ maps the Zariski tangent space $\mathrm{Z}_p$ to itself.\\
    To this end, let $v \in \mathrm{Z}_p$ and $F \in \mathcal{M}$ be arbitrary. Because $F$ is a magnetomorphism, the differential of $F$ and the Lorentz force commute, so that
    \[
    d_p F \cdot Y_p( v) = Y_p (d_p F \cdot v) = Y_p(v) \,\, , 
    \]
    where the second equation follows from $v \in \mathrm{Z}_p$ and the definition of the Zariski tangent space in \eqref{eq: totally magnetic submfds - Zariski space}. Because $F \in \mathcal{M}$ was arbitrary, \eqref{eq: totally magnetic submfds - Zariski space} again shows that $Y_p (v) \in \mathrm{Z}_p \,$. This finishes the proof.
\end{proof}

\begin{proof}[Proof of \Cref{prop: totally magnetic submfds - intersections}]
   Let $p \in N = N_1 \cap N_2$ be arbitrary and observe that $\exp^M_p : B_\e(0) \overset{\sim}{\rightarrow} B_\e(p)$ maps $B_\e(0) \cap T_p N_1 \cap T_p N_2$ bijectively to $B_\e(p) \cap N_1 \cap N_2 \,$. Thus the connected components of $N$ are totally geodesic submanifolds. It moreover shows that the tangent space of the connected component containing $p$ is given by $T_p N_1 \cap T_p N_2 \,$.
   Now, every magnetic geodesic of $(M,g,\sigma)$ starting at $p \in N$ with initial velocity in $T_p N_1 \cap T_p N_2$ stays in both $N_1$ and $N_2$ for a short time and hence in the connected component of $N=N_1 \cap N_2$ containing $p \,$.
\end{proof}


\subsection{Applications to Ellipsoids}
\label{subsection: totally magnetic submfds - Ellipsoids}

Following the notation of \Cref{subsection: magnetomorphism group - Ellipsoids}, we write $E(\mathbf{a}) \in \IC^n$ for the complex ellipsoid associated to the sequence
\[
 \underbrace{a_1 = \ldots = a_1}_{\ell_1\text{-times}} < \underbrace{a_2 = \ldots = a_2}_{ \ell_2\text{-times}} < \ldots < \underbrace{a_k = \ldots = a_k}_{\ell_k \text{-times}} \,\, ,
\]
where $\mathbf{a}_j := (a_j,\ell_j) \comma j=1,\ldots , k \, $, and $\mathbf{a} = (\mathbf{a}_1,\ldots , \mathbf{a}_k) \,$. We endow $E(\mathbf{a})$ with the pullback of the Euclidean metric and the pullback of the canonical symplectic form as magnetic form.
\\

\noindent For each $j=1,\ldots , n$ consider the unitary matrix
\begin{align*}
    U_j := \mathrm{diag}(1,\ldots , 1, -1,1,\ldots , 1) \in \Unitary(n)
\end{align*}
with $-1$ at the $j$-th position. $U_j$ restricts to a magnetomorphism of the ellipsoids $E(\mathbf{a}) $ whose fixed points have $j$-th component equal to zero. Let $J \subseteq \{1,\ldots , n\}$ be a subset. \Cref{prop: totally magnetic submfds - fixed point set} implies that
\[
N_J := \mathrm{Fix}(\{U_j\}_{j \in J}) = \set{(z_1,\ldots , z_n) \in E(\mathbf{a})}{z_j = 0 \quad \forall \, j \in J}  
\]
is a totally magnetic submanifold of $E(\mathbf{a}) \,$. Multiplying $N_J$ by unitary matrices of the form
\[
U = \mathrm{diag}(U_1,\ldots , U_k) \comma \quad U_1 \in \Unitary(\ell_1) \comma \ldots \comma U_k \in \Unitary(k) \,\, ,
\]
which we know by \Cref{prop: magnetomorphism group - Ellipsoids} restrict to magnetomorphisms of the ellipsoid, we obtain new totally magnetic submanifolds of $E(\mathbf{a}) \,$. One readily sees that every subset
\begin{equation}
\label{eq: totally magnetic submfds - Ellipsoids}
E(\mathbf{a}) \,\cap \, (V_1 \oplus \ldots \oplus V_k) \comma \quad V_j \subseteq \IC^{\ell_j} \text{ complex linear subspace }  \comma \, j=1,\ldots , k \,\, ,
\end{equation}
can be obtained in this way. We have thus proven the following result.

\begin{cor}
\label{cor: totally magnetic submfds - Ellipsoids}
Let $V_1 \subseteq \IC^{\ell_1} , \ldots , V_k \subseteq \IC^{\ell_k}$ be complex linear subspaces. Then
\[
E(\mathbf{a}) \,\cap \, (V_1 \oplus \ldots \oplus V_k) 
\]
is a totally magnetic submanifold of $E(\mathbf{a}) \,$.
\end{cor}

In the case $k=1 \,$, that is $E(\mathbf{a}) = \SS^{2n-1} \,$, it was proven in \cite[Cor. 1.5]{ABM}
that all closed totally magnetic submanifolds are the intersection of the ellipsoid with a complex linear subspace. Based on this, we conjecture the following.

\begin{conj}
\label{conj: totally magnetic submfds - Ellipsoids}
Every closed totally magnetic submanifold of $E(\mathbf{a})$ is of the form \eqref{eq: totally magnetic submfds - Ellipsoids}.
\end{conj}


\subsection{Totally Magnetic Submanifolds of Hypersurfaces in Euclidean Space}
\label{subsection: totally magnetic submfds - hypersurfaces in Euclidean Space}

In view of the \Cref{conj: totally magnetic submfds - Ellipsoids}, we give a necessary condition for totally magnetic submanifolds of ellipsoids and more generally hypersurfaces in Euclidean space.

 We work in the setting of \Cref{subsection: magnetic geodesic equation - Application to Ellipsoids}, that is $\Sigma = f^{-1}(c) \subseteq \IC^n = \IR^{2n}$ is a regular level set of a smooth function $f : \IR^{2n} \rightarrow \IR \,$. We denote by $i : \Sigma \hookrightarrow \IR^{2n}$ the inclusion and consider the magnetic system $(\Sigma, \, i^*g_{\mathrm{euc}}  , \, i^* \omegacan ) \,$. As previously, we also write $\langle \,\cdot\comma \cdot\,\rangle_{\IR} = g_{\mathrm{euc}}$ for the Euclidean inner product on $\IR^{2n} \,$.

\begin{lem}
\label{lem: totally magnetic submfds - Euclidean space criterion}
A totally geodesic submanifold $S$ of $(\Sigma \comma i^* \,g_{\mathrm{euc}})$ is a totally magnetic submanifold of
$(\Sigma \comma i^* \,g_{\mathrm{euc}} \comma i^* \,\omegacan)$ if and only if 
\begin{align}
\label{eq: totally magnetic submfds - Euclidean space criterion}
    \i \, v - \frac{\Rproduct{\i \, v}{\nabla f (x)}}{|\nabla f (x)|^2} \,\, \nabla f (x) \in T_x S \qquad \Forall \, v \in T_x S \comma \, x \in S \,\, .
\end{align}
\end{lem}

\begin{proof}
    Recall that the Lorentz force of the magnetic system $(\IR^{2n} , g_{\mathrm{euc}} , \omegacan)$ is just multiplication by $\i$. By Formula \eqref{eq: magnetic geodesic eq - Ytilde gammadot}, the Lorentz force $Y$ of the magnetic system $(\Sigma , \, i^* \,g_{\mathrm{euc}} , \, i^* \,\omegacan)$ is hence given by
    \begin{align*}
       T\Sigma \ni (x,v) \mapsto Y_x(v) =  \i \, v - \frac{\Rproduct{\i \, v}{\nabla f (x)}}{|\nabla f (x)|^2} \,\, \nabla f (x) \,\, .
    \end{align*}
    Now recall from \Cref{t: totally magnetic submfds - characterization totally magnetic from ABM} that $S$ is a totally magnetic submanifold iff $TS$ is $Y$-invariant.
\end{proof}

\begin{rem}
\label{rem: totally magnetic submfds - i grad f in T Sigma}
Clearly $\i \, \nabla f (x) \in \{\nabla f (x) \}^{\perp} = T_x \Sigma$ for every $x \in \Sigma$.
\end{rem}

\begin{prop}
\label{prop: totally magnetic submfds of regular level sets}
Suppose $S$ is a totally magnetic submanifold of $(\Sigma \comma i^* \,g_{\mathrm{euc}} \comma i^* \,\omegacan) \,$. Then for every $x \in S$ the real linear subspace $T_x S + \IR \cdot \nabla f (x) + \IR \cdot \i \, \nabla f (x) \subseteq \IR^{2n}$ is a complex linear subspace. Moreover, for every $x \in S$ it holds
\begin{enumerate}[label=(\roman*)]
    \item\label{it: totally magnetic submfds - dim(S) odd} $\dim(S)$ is odd \,\, $\Longleftrightarrow \,\, \i \, \nabla f (x) \in T_x S$ \\
    \item\label{it: totally magnetic submfds - dim(S) even} $\dim(S)$ is even \hspace*{1mm}$\Longleftrightarrow \,\, \i \, \nabla f (x) \notin T_x S \,\, \Longleftrightarrow \,\, T_x S$ is a complex linear subspace of $\IR^{2n}$.
\end{enumerate}
\end{prop}

\begin{proof}
    Looking at \eqref{eq: totally magnetic submfds - Euclidean space criterion}, it is obvious that $\i \, T_x S \subseteq T_x S + \IR \cdot \nabla f (x)$ for every $x \in S$. Hence $V_x := T_x S + \IR \cdot \nabla f(x) + \IR \cdot \i \, \nabla f (x)$ is invariant under multiplication by $\i$ and therefore a complex linear subspace.\\
    If $\, \i \,  \nabla f (x) \in T_x S$, then $V_x = T_x S \oplus \IR \cdot \nabla f (x)$ is complex linear, hence $T_x S$ is odd dimensional. Conversely, if $\, \i \, \nabla f (x) \notin T_x S$, then we have the direct sum decomposition
    \begin{align}
    \label{eq: totally magentic submfds - V_x direct sum}
    V_x = T_x S \,\oplus\, \IR \cdot \nabla f (x) \,\oplus\, \IR \cdot \i \, \nabla f (x)
    \end{align}
    because both $\, \i \, \nabla f (x)$ and $T_x S$ are contained in $T_x \Sigma \,$. We want to show that $T_x S$ is a complex linear subspace. Let $v \in T_x S$ be arbitrary. By \eqref{eq: totally magnetic submfds - Euclidean space criterion}, it holds $\, \i \, v = v_1 + a \, \nabla f (x)$ for some $v_1 \in T_x S$ and $a \in \IR \,$. Multiply this by $\i$ to obtain
    \begin{align*}
        T_x S \ni -v = \i \, v_1 + a \, \i \, \nabla f (x) \,\, .
    \end{align*}
  Since $\i \, v_1 \in T_x S \oplus \IR \cdot \nabla f (x)$ by \eqref{eq: totally magnetic submfds - Euclidean space criterion} again, from the direct sum decomposition \eqref{eq: totally magentic submfds - V_x direct sum} we deduce that $a = 0$ and hence $\, \i \, v = v_1 \in T_x S \, $. As $v $ was arbitrary, indeed $T_x S$ is a complex linear subspace.
\end{proof}

\begin{cor}
\label{cor: totally magnetic sufmfds - 1-dim classification}
The connected $1$-dimensional totally magnetic submanifolds of $(\Sigma, \, i^*g_{\mathrm{euc}} , \, i^*\omegacan)$ are precisely the images of embedded curves $\gamma$ that are both geodesics of $(\Sigma, \, i^*g_{\mathrm{euc}})$ and integral curves of $\i \, \frac{\nabla f}{|\nabla f|} \,$.
\end{cor}

\begin{proof}
    Given a $1$-dimensional totally magnetic submanifold $S$, it follows from \Cref{prop: totally magnetic submfds of regular level sets} \ref{it: totally magnetic submfds - dim(S) odd} that $\i \, \nabla f$ is tangent to $S$. So the maximal integral curve $\gamma$ of $\i \, \frac{\nabla f}{|\nabla f|}$ starting at some fixed choice $p_0 \in S$ is a parametrization of $S$ that moreover is a unit-speed geodesic since $S$ is also a totally geodesic submanifold.

    Conversely, suppose $S$ is parametrized by the integral curve $\gamma$ of $\i \, \frac{ \nabla f}{|\nabla f|}$ which moreover is a geodesic in $\Sigma \,$. Then $S$ is a totally geodesic submanifold of $\Sigma$ and one easily verifies \eqref{eq: totally magnetic submfds - Euclidean space criterion}, so that $S$ is a totally magnetic submanifold by \Cref{lem: totally magnetic submfds - Euclidean space criterion}.
\end{proof}
